Towards Massive MIMO 2.0: Understanding spatial correlation, interference suppression, and pilot contamination

Since the seminal paper by Marzetta from 2010, Massive MIMO has changed from being a theoretical concept with an infinite number of antennas to a practical technology. The key concepts are adopted in 5G and base stations (BSs) with $M=64$ full-digital transceivers have been commercially deployed in sub-6\,GHz bands. The fast progress was enabled by many solid research contributions of which the vast majority assume spatially uncorrelated channels and signal processing schemes developed for single-cell operation. These assumptions make the performance analysis and optimization of Massive MIMO tractable but have three major caveats: 1) practical channels are spatially correlated; 2) large performance gains can be obtained by multicell processing, without BS cooperation; 3) the interference caused by pilot contamination creates a finite capacity limit, as $M\to\infty$. There is a thin line of papers that avoided these caveats, but the results are easily missed. Hence, this tutorial article explains the importance of considering spatial channel correlation and using signal processing schemes designed for multicell networks. We present recent results on the fundamental limits of Massive MIMO, which are not determined by pilot contamination but the ability to acquire channel statistics. These results will guide the journey towards the next level of Massive MIMO, which we call ``Massive MIMO 2.0''.

==> SectionIX.tex <==
%!TEX root = TCOM.tex

%\section{What are the potential benefits of cooperation between BSs?}
Until now, we have considered a system in which each BS processes individually the signals to/from its own UEs. A radically different way of deploying Massive MIMO is to let the BSs cooperate to jointly process the signals to/from UEs. Different network configurations with various degrees of cooperation can be envisioned. In this article, the following two are considered. 
\begin{itemize}
\item A \emph{fully cooperative} Massive MIMO network in which the BSs share the CSI of the UEs as well as their data through backhaul links. This is a form of network MIMO \cite{Gesbert2010a,Bjornson2013d} that uses TDD and where the number of antennas per UE is large. 
\item A \emph{partially cooperative} Massive MIMO network in which the BSs share data but only has access to \emph{local CSI} that each BS can estimate locally \cite{Bjornson2013d}. %In the Massive MIMO literature, 
This concept is called \emph{cell-free} Massive MIMO \cite{Ngo2017b}. 
%Although the cell-free notion is only used for this network configuration in the Massive MIMO literature, we notice that in both configurations there are no longer cells.
\end{itemize}
Suppose both networks consist of $L$ BSs, each equipped with $M$ antennas, that jointly serve $KL$ UEs that can be located anywhere in the coverage area.
%The cell-free extension of our canonical Massive MIMO network consists of a single-cell in which $L$ spatially distributed BSs, each equipped with $M$ antennas, process the signals of $KL$ UEs by using a synchronous TDD protocol. 
With a slight abuse of notation, we maintain the double index format (used so far) to refer to UEs in the network; that is, $\vect{h}_{jk}^{n} \sim \CN ( \vect{0}, \vect{R}_{jk}^{n})$ is the channel vector from UE~$k$ in the \emph{hypothetical} cell $j$ to BS $n$. We thus call $\vect{v}_{jk}^{n}$ the combining vector used at BS $n$ to process the signal of UE $k$ in the hypothetical cell $j$ and define 
\begin{align}
{\bf v}_{jk} &\triangleq \left[{({\bf v}_{jk}^1)}^{\Ttran},{({\bf v}_{jk}^2)}^{\Ttran},\ldots,{({\bf v}_{jk}^L)}^{\Ttran}\right]^{\Ttran}\in \mathbb{C}^{LM}.
\end{align}

\begin{figure}[t!]
\begin{center}
\begin{overpic}[unit=1mm,width=1\columnwidth]{figures/section7_figure19_ULSE_Cfv1.eps}
\put(21,45){\scriptsize MR}
\put(54,30){{\color{red}\scriptsize M-MMSE}}
\end{overpic}
\end{center}
\caption{CDF of the UL SE per UE with different Massive MIMO architectures when $M=100$ and $f=1$ for the multicell setup in Fig.~\ref{figure_network_layout}. The cell-free Massive MIMO curve with MR refers to the two-layer LSFD scheme in \cite{VanChien-18}.} \label{CDF_of_different_configuration}
\end{figure}
 \begin{figure*}
\begin{equation} \label{eq:uplink-SINR-expression-forgetbound-cf}
\begin{split}
\underline{\gamma}^{\mathrm{ul}}_{jk} = \frac{  \bigg| \sum\limits_{n=1}^L(a_{jk}^n)^*\mathbb{E}\{ {(\vect{v}_{jk}^{n})}^{\Htran} \vect{h}_{jk}^{n}  \} \bigg|^2  }{ 
\sum\limits_{l=1}^{L} \sum\limits_{i=1}^{K_l}   \mathbb{E} \left\{  \bigg| \sum\limits_{n=1}^L(a_{jk}^n)^* {(\vect{v}_{jk}^{n})}^{\Htran}  \vect{h}_{li}^{n} \bigg|^2 \right\}
-  \bigg| \sum\limits_{n=1}^L(a_{jk}^n)^*\mathbb{E}\{ {(\vect{v}_{jk}^{n})}^{\Htran}  \vect{h}_{jk}^{n}  \} \bigg|^2 + \frac{\sigma^2_{\rm {ul}}}{\rho_{\rm {ul}}} \sum\limits_{n=1}^L|{a_{jk}^n}|^2\mathbb{E}\{ \|  \vect{v}_{jk}^{n}   \|^2 \}  }.
\end{split}
\end{equation}
\hrule
\end{figure*}

In a fully cooperative Massive MIMO network, the entire network acts as being a single cell. If the MMSE estimator is used locally at each BS,  the optimal ${\bf v}_{jk}$ that maximizes the SINR expression in Theorem \ref{theorem:uplink-SE} is
\begin{equation} \label{eq:MMSE-combining-fully-cooperative}
\vect{v}_{jk}^{\rm{MMSE}} =   \Bigg(  \sum\limits_{l=1}^L\sum\limits_{i=1}^K \widehat{\bf h}_{li}\widehat{\bf h}_{li}^{\Htran} + \vect{Z}  \Bigg)^{\!-1}    \widehat{\bf h}_{jk}
\end{equation}
with ${\bf Z} = {{\rm{diag}}\left({\bf Z}_1,{\bf Z}_2,\ldots,{\bf Z}_L\right)} \in \mathbb{C}^{LM\times LM}$ being block-diagonal and $\widehat{\bf h}_{jk} = \big[{(\widehat{\bf h}_{jk}^1)}^{\Ttran},{(\widehat{\bf h}_{jk}^2)}^{\Ttran},\ldots,{(\widehat{\bf h}_{jk}^L)}^{\Ttran}\big]^{\Ttran}\in \mathbb{C}^{LM}$. 
This is MMSE combining; we drop the multi-cell notion since there are no cells. 
%Although MMSE combining in \eqref{eq:MMSE-combining-fully-cooperative} is optimal, we notice that a fully cooperative network in which the BSs share their channel estimates is hard to achieve in practice since channels change rapidly over time.

%Since there are no cells, the double index notation used so far is no longer needed. We thus call $\vect{h}_{k}^{j} \sim \CN ( \vect{0}, \vect{R}_{k}^{j})$ the channel vector from UE~$k$ to BS~$j$ and assume that is independent from the channel vectors of other BSs (since they are spatially distributed). Hence, the overall channel ${\bf h}_{k}= [{({\bf h}_{k}^{1})}^{\Ttran},\ldots,{({\bf h}_{k}^{L})}^{\Ttran}]^{\Ttran}\in \mathbb{C}^{ML}$ has a block-diagonal correlation matrix $\vect{R}_{k} = {\rm{diag}}\left(\vect{R}_{k}^1,\ldots,\vect{R}_{k}^L\right) \in \mathbb{C}^{LM\times LM}$. We let $\bphiu_{k} \in \mathbb{C}^{\taupu}$ denote the pilot sequence used by UE~$k$ and let $\Pu_{k} \subset \{1,\ldots, K\}$ be the group of UEs that utilize the same pilot as this UE. If the pilot is transmitted with power $\rho_{\rm{ul}}$, the MMSE estimate of $\vect{h}_{k}^{j}$ is 
%\begin{equation} \label{eq:MMSEestimator_h_jli_v1}
%\widehat{\vect{h}}_{k}^{j}  = \vect{R}_{k}^{j} \big(\Psiv_{k}^{j}\big)^{-1}  \left(\vect{h}_{k}^{j} + \sum\limits_{i\in \mathcal{P}_k}\vect{h}_{i}^{j}+\frac{1}{\tau_p\sqrt{\rho_{\rm{ul}}}}\vect{N}_{j}^{p}\bphiu_{i}\right)
%\end{equation}
%where $\Psiv_{k}^{j} =  \sum_{i\in \Pu_{k} }\vect{R}_{i}^{j}  +  \frac{1}{\tau_p}\frac{\sigm\alpha_{\rm{ul}}^2}{\rho_{\rm{ul}}}  \vect{I}_{M}$. In a cell-free Massive MIMO network, BS~$j$ uses $\widehat{\vect{h}}_{k}^{j}$ to process the signal from UE~$k$ using a receive combining vector $\vect{v}_k^j\in \mathbb{C}^{M}$. This produces the scalar ${(\vect{v}_k^j)}^{\Htran}\vect{y}_j$ with
%\begin{align} \label{eq:uplink-signal-model_cf}
%\vect{y}_j = \vect{h}_{k}^{j} s_{k} + \sum_{i=1,i\ne k}^{KL} \vect{h}_{i}^{j} s_{i} + \vect{n}_{j}
%\end{align}


In a cell-free Massive MIMO network, the optimal MMSE combining in \eqref{eq:MMSE-combining-fully-cooperative} cannot be implemented since each BS can only use its own local CSI. Alternative combining schemes are therefore needed. A potential solution is the so-called \emph{large-scale fading decoding} (LSFD) strategy, which was originally proposed in \cite{ashikhmin2012pilot}. In its more recent form \cite{Adhikary2017a,VanChien-18}, it consists of two layers. In the first layer, each BS locally applies an arbitrary receive combiner to obtain \emph{local} estimates of each UEs' data; for example, BS $n$ computes $\widehat s_{jk}^{\,n} = {(\vect{v}_{jk}^n)}^{\Htran} \vect{y}_{j}$ as a local estimate of $s_{jk}$. The local estimates $\{\widehat s_{jk}^{\,n}: \forall n\}$ are then gathered at a central unit where they are linearly combined to obtain $\sum_{n=1}^L a_{jk}^n\widehat s_{jk}^{\,n}$, which is eventually used to decode $s_{jk}$. The coefficients $\{a_{jk}^n:\forall n\}$ used in the second stage can be optimized to suppress the residual interference from the first layer, but only channel statistics can be utilized since no CSI is shared over the network. In \cite{VanChien-18}, the authors proposed to maximize the UatF bound in Theorem \ref{theorem:uplink-capacity-forgetbound}. For any choice of the combining vectors $\{\vect{v}_{jk}^{\,n}:\forall n\}$ and LSFD coefficients $\{{a}_{jk}^{\,n}:\forall n\}$, the UatF bounding technique yields $\underline{\mathacr{SE}}^{\mathrm{ul}}_{jk}= \frac{\tau_u}{\tau_c} \log_2  ( 1 + \underline{\gamma}^{\mathrm{ul}}_{jk} )$ [bit/s/Hz] with $\underline{\gamma}^{\mathrm{ul}}_{jk}$ given in \eqref{eq:uplink-SINR-expression-forgetbound-cf}.

%
%
%
%\begin{equation} \label{eq:uplink-SINR-expression-forgetbound}
%\begin{split}
%\underline{\gamma}^{\mathrm{ul}}_{k} = \frac{  \bigg| \mathbb{E}\bigg\{ \sum\limits_{j=1}^La_{k}^j{(\vect{v}_{k}^{j})}^{\Htran} \vect{h}_{k}^{j}  \bigg\} \bigg|^2  }{  \sum\limits_{i=1}^{KL}   \mathbb{E} \bigg\{ \bigg| \sum\limits_{j=1}^La_{k}^j{(\vect{v}_{k}^{j})}^{\Htran}\vect{h}_{j}^{j} \bigg|^2 \bigg\}
%-  \bigg| \mathbb{E}\bigg\{ \sum\limits_{j=1}^La_{k}^j{(\vect{v}_{k}^{j})}^{\Htran} \vect{h}_{k}^{j}  \bigg\} \bigg|^2 + \frac{\sigma^2_{\rm {ul}}}{\rho_{\rm {ul}}} \mathbb{E}\bigg\{ \sum\limits_{j=1}^La_{k}^j{(\vect{v}_{k}^{j})}^{\Htran} \vect{v}_{k}^{j}  \bigg\}  }.
%\end{split}
%\end{equation}
%To obtain a practically implementable form of cell-free Massive MIMO, each BS should only employ CSI that can be locally obtained, to avoid the cumbersome exchange of CSI between BSs. In this respect, MR combining with $\vect{v}_{jk} = \widehat{\vect{h}}_{jk}^{j}$ is the most suitable scheme \cite{Ngo2017b}. 
The LSFD coefficients that maximize \eqref{eq:uplink-SINR-expression-forgetbound} with MR combining, i.e., $\vect{v}_{jk}^{n} = \widehat{\vect{h}}_{jk}^{n}$, are given by ${\vect{a}}_{jk} = {\vect{C}}_{jk}^{-1}{\vect{b}}_{jk}$ 
where ${\vect{b}}_{jk}\in \mathbb{C}^{L}$ has elements $\left[{\vect{b}}_{jk}\right]_{n} = \tr \! \left( \vect{R}_{jk}^{n} {(\Psiv_{jk}^{n})}^{-1}\vect{R}_{jk}^{n} \right)$, ${\vect{C}}_{jk} = \sum\limits_{l\in \mathcal P_j}{\vect{b}}_{lk}{\vect{b}}_{lk}^{\Htran} + {\vect{\Lambda}}_{jk}$ 
and ${\vect{\Lambda}}_{jk}\in \mathbb{C}^{L\times L}$ is the diagonal matrix given by
\begin{align}\notag
\left[{\vect{\Lambda}}_{jk}\right]_{nn} &= \frac{\sigma_{\rm{ul}}^2}{\rho_{\rm{ul}}} \tr \! \left( \vect{R}_{jk}^{n} {(\Psiv_{jk}^{n})}^{-1}\vect{R}_{jk}^{n} \right) \\&+\sum\limits_{l=1}^{L}\sum\limits_{i=1}^{K} \tr \!\left( \vect{R}_{li}^{n}  \vect{R}_{jk}^{n} {(\Psiv_{jk}^{n})}^{-1}   \vect{R}_{jk}^{n} \right).
\end{align}



Fig.~\ref{CDF_of_different_configuration} compares the CDFs of the UL SE per UE for Massive MIMO and the two cooperative networks. We consider MR and MMSE combining, but omit MMSE in the cell-free Massive MIMO case since it is not implementable without CSI exchange. The cell-free Massive MIMO curve with MR uses the two-layer LSFD scheme described above. Fig.~\ref{CDF_of_different_configuration} shows that a fully cooperative network MIMO system can give substantial gains over conventional Massive MIMO (with no cooperation among BSs), but only when MMSE combining is used. In case of MR combining, a network MIMO system does not bring any benefit compared to Massive MIMO; by looking closely at the results it is the latter that performs marginally better, simply because distant BSs  contribute with more interference than signal power in network MIMO with MR combining.
This can be handled by LSFD, as demonstrated by the cell-free curve in Fig.~\ref{CDF_of_different_configuration}, but this leads to essentially the same SE as with Massive MIMO, i.e., it is optimal to only use the received signal from the BS with the best channel. 
%This effect can be mitigated by using the optimized LSFD framework, but only marginally. Indeed, the result show that it allows to achieve the same performance of non-cooperative network. 

In summary, it seems that the benefits of cooperation among BSs can only be achieved if the BSs are jointly suppressing interference. This usually requires the BSs to share instantaneous CSI so that a strong interference term received at one BS can be cancelled by an equally strong interference term with the opposite phase at another BS. Maybe some new clever cooperation schemes can be developed to implement this without requiring instantaneous CSI sharing, but these will probably be very sensitive to phase synchronization errors \cite[Section 4.2.2]{Bjornson2013d}.
% interference suppression schemes are employed. This requires the BSs to share instantaneous CSI. Since this is hard to achieve in practice, it is unclear to what extent Massive MIMO can benefit from cooperation. 
 Further research activities are required to fully understand these issues.


%but we know that this is not the optimal choice when the BSs have multiple antennas. Inspired by the OBE combining in \eqref{eq:OBE}, recently \cite{SBH-GC-18} showed that its cell-free extension takes the form  
%\begin{align}\label{eq:OBE-distributed}
%\vect{v}_{jk}^{\rm{CF-OBE}} & = {\big({{\bf U}}_{j}\big)}^{-1} \left(\sum_{i\in \mathcal{P}_k}c_{ki}\widehat{\bf {h}}_{i}^j \right)
%\end{align}
%where ${{\bf U}}_{j} = \sum\limits_{i=1}^{KL} {\vect{R}}_{i}^{j}+\frac{\sigma^2_{\rm {ul}}}{\rho_{\rm {ul}}}{\bf I}_M$ and the scalar coefficients are computed as $c_{ki} = [\vect{c}_k]_i$ with $\vect{c}_k = \big(\vect{\Theta}+{\vect{I}_{|\mathcal{P}_k|}}\big)^{-1}\vect{e}_k$ where $ [\vect{\Theta}]_{li} = \tr \big({\bf R}_{i}^j (\Psiv_{k}^{j})^{-1}   {\bf R}_{l}^j({{\bf U}}_{j})^{-1}\big)$ $\forall l,i \in \mathcal{P}_k$.

%\begin{figure}[t!]\vspace{-0.5cm}
%\begin{center}
%\subfloat[CDF of the average channel gain for a Massive MIMO network, i.e., $\beta_{jk}=\frac{1}{M}{\trace \big(\vect{R}_{jk}^j}\big)$, and cell-free Massive MIMO, i.e., $\beta_k=\frac{1}{M}{\trace \big(\vect{R}_k}\big)$.]{\label{figure:ul_se_vs_antennas_CorrelatedChannels}
%\begin{overpic}[unit=1mm,width=.52\columnwidth]{figures/section7_figure19a_ULSE_Cf.eps}
%\end{overpic}} 
%\subfloat[UL sum SE with different combining schemes.]{\label{figure:dl_se_vs_antennas_CorrelatedChannels}
%\begin{overpic}[unit=1mm,width=.52\columnwidth]{figures/section7_figure19b_ULSE_Cf.eps}
%\put(52,30){{\color{red}\scriptsize M-MMSE}}
%\put(33,33){{\color{blue}\scriptsize OBE}}
%\put(31,53){{\scriptsize MR}}
%\end{overpic}} 
%\end{center} \vskip-6mm
%\caption{Performance evaluation of a canonical Massive MIMO network and a cell-free Massive MIMO system. The network setup is of Fig.~\ref{figure_network_layout} with $M=64$, $K=8$ and pilot reuse factor $f=1$.}\label{se_cf}\vspace{-0.8cm}
%\end{figure}


